LONGCODEU: Benchmarking Long-Context Language Models on Long Code Understanding

Current advanced long-context language models offer great potential for real-world software engineering applications. However, progress in this critical domain remains hampered by a fundamental limitation: the absence of a rigorous evaluation framework for long code understanding. To gap this obstacle, we propose a long code understanding benchmark LONGCODEU from four aspects (8 tasks) to evaluate LCLMs' long code understanding ability required for practical applications, including code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long code documentation understanding. We evaluate 9 popular LCLMs on LONGCODEU (i.e., 6 general models and 3 code models). Our experimental results reveal key limitations in current LCLMs' capabilities for long code understanding. Particularly, the performance of LCLMs drops dramatically when the long code length is greater than 32K, falling far short of their claimed 128K-1M context windows. In the four aspects, inter-code unit relation understanding is the most challenging for LCLMs. Our study provides valuable insights for optimizing LCLMs and driving advancements in software engineering.

==> 3-Experimental_Setup.tex <==
\section{Experimental Setup}






==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/1-Introduction.tex <==
\section{Introduction}
\label{Introduction}


\begin{figure}[t]
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-5mm}
\includegraphics[width=\columnwidth]{latex/figure/Introduction_example.pdf}
\caption{Examples of a synthetic long code with independent functions and a real-world long code with non-standalone functions. Dependencies are highlighted.}
\label{figure: benchmark comprison}
% \vspace{-0.4cm}
\end{figure}



Recent advances in long-context language models (LCLMs) like Gemini-1.5 \cite{team2024gemini} and GPT-4o \cite{GPT-4o}, which support context windows exceeding hundreds of thousands of tokens, offer unprecedented potential for real-world software engineering applications. These models promise transformative improvements in related downstream tasks, such as repository-level code generation \cite{zhang2024codeagent, bi2024iterative}, real-world GitHub issues resolution\cite{jimenez2023swe}, and long code summarization \cite{dhulshette2025hierarchical}. However, progress in this critical area remains hampered by a fundamental limitation: \textbf{the lack of rigorous evaluation frameworks for long code understanding}—a capability essential for real-world software development tools that require accurate code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long code documentation understanding in code repositories.








Current benchmarks generally fall into two categories, which face five fundamental limitations that hinder comprehensive evaluation of LCLMs' long code understanding capabilities.  
The first category includes studies such as RepoQA \cite{liu2024repoqa}, whose task design has insufficient diversity like only focusing on needle function search. While these evaluations are useful, \ding{182} \textbf{they do not capture the real-world full range of code understanding capabilities} needed for practical coding scenarios. Additionally, benchmarks like L-Eval \citet{an2023eval} further compound these limitations by using synthetic ``long code'' through a simple joining of independent code snippets. \ding{183} This approach \textbf{overlooks the natural dependencies between code segments}, as shown in Figure~\ref{figure: benchmark comprison}. 
\ding{184} These studies also face issues with \textbf{data contamination}. They neither enforce temporal constraints on code release dates nor address potential model pre-exposure through evaluating on previously published datasets. \ding{185} Their maximum supported context length of 36.5K tokens also \textbf{falls far short of stress-testing the claimed 128K-1M context windows of modern LCLMs}.
The second category includes benchmarks like Long Code Arena \cite{bogomolov2024long}, LongBench \cite{bai2023longbench}, SWE-bench \cite{jimenez2023swe}, and DevEval \cite{li2024deveval}, which evaluate long-context understanding based on performance in downstream tasks. 
\ding{186} However, these benchmarks \textbf{entangle code understanding with other task-specific challenges} like code generation and bug fixing.
This makes it hard to determine whether performance limitations are due to a lack of code understanding or other factors.


To address these limitations, we propose \method, a benchmark designed to isolate and comprehensively evaluate LCLMs' capacity to understand and reason about real-world, dependency-rich, long code contexts. Our benchmark offers the following key features:
\begin{itemize}[topsep=0pt,noitemsep] 
\item[$\bullet$] \textbf{Comprehensive Tasks stem from Practical Applications.} We evaluate LCLMs from four aspects (8 tasks) to evaluate the LCLMs' long code understanding capability required for practical applications, including code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long documentation understanding.


\item[$\bullet$] \textbf{Extra-long Code Context.} Each task contains around 500 gathered long codes. The lengths of examples change in 0$\sim$8K, 8$\sim$16K, 16$\sim$32K, 32$\sim$64K, and 64$\sim$128K following the normal distribution, which far exceeds the maximum length of 36.5K supported by existing benchmarks \cite{an2023eval}.


\item[$\bullet$] \textbf{Real-world Repository.} The benchmark is collected from real-world code repositories. Long code consists of one or more real code file contents, instead of being composed of multiple independent code units like current benchmarks \cite{liu2024repoqa}. 


\item[$\bullet$] \textbf{Reducing Data Contamination.} We collect up-to-date code repositories that are created after 2024-06 from GitHub\footnote{https://github.com/}, which are later than most prevailing LCLMs' cut-off dates thus reducing the risk of data contamination.

\end{itemize}


We evaluate 9 popular LCLMs, which contain 6 general models (\ie GPT-4o \cite{GPT-4o}, Claude-3.5-Sonnet \cite{claude-3.5}, Gemini-1.5-Flash \cite{team2024gemini}, DeepSeek-V2.5 \cite{bai2023longbench}, Mistral-v0.3 \cite{jiang2023mistral}, and Phi-3.5 \cite{abdin2024phi} ) and 3 code models (\ie DeepSeek-Coder-V2 \cite{bai2023longbench},  Qwen2.5-Coder \cite{hui2024qwen2}, CodeLlama \cite{roziere2023code}) on \method. 
The experimental results reveal key limitations in current LCLMs' capabilities for long code understanding. Especially, \textbf{LCLMs’ performance drops dramatically when the long code length is greater than 32K, falling far short of their claimed context windows such as 128K-1M tokens}. 
In the four aspects, \textbf{inter-code unit relation understanding is the most challenging for LCLMs.}
Our findings provide valuable insights for optimizing LCLMs and driving advancements in software engineering.



\begin{table*}[htbp]
  \centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-5mm}
\caption{The comparison between existing benchmarks and \method. \#Num is the abbreviation of number. \#Div Tasks refers to diverse tasks. \#High Disp represents high dispersion.  \#Max-L and \#Avg-L mean the maximum length and the average length of long code. \#Trunk-L means whether each example has the length label. \#Doc refers to documentation related to repositories. \#Task represents the number of tasks (\ie examples).}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{Benchmark} & \multicolumn{3}{c|}{Comprehensive Code Tasks}              & \multicolumn{3}{c|}{Extra-long Data} & \multicolumn{3}{c|}{Real-world Repository} & \multicolumn{1}{c|}{Reduce Data Leaking} & \multicolumn{1}{c}{Data Scale} \\
          & \multicolumn{1}{c}{\#Num} &  \multicolumn{1}{c}{\#Div Tasks}  & \multicolumn{1}{c|}{\#High Disp} & \multicolumn{1}{c}{\#Max-L} & \multicolumn{1}{c}{\#Avg-L} & \multicolumn{1}{c|}{\#Length-L} & \multicolumn{1}{c}{Code} & \multicolumn{1}{c}{\#Doc}  & \multicolumn{1}{c|}{\#Num} & \multicolumn{1}{c|}{Data Time}  & \multicolumn{1}{c}{\#Task} \\
    \midrule
    \multicolumn{12}{l}{\textit{\textbf{The second category benchmarks (Only some benchmarks are listed)}}} \\
    \midrule
    LongBench~[\citenum{bai2023longbench}]    &  2 &  \ding{55} &  \ding{55}  &  --  & 0.4K &  \ding{55}  &  Function &  \ding{55} &  -- &  2023.02--2023.08     &  1,000  \\
    LC-Arena~[\citenum{bogomolov2024long}]   &  6 &  \ding{55} &  \ding{55}  & -- & -- & \ding{55}   & File  & \ding{55}  & 62  &  2023.01--2024.05  & --   \\
    LONGPROC~[\citenum{ye2025longproc}]   & 1  & \ding{55}  &  \ding{51}  & -- & 2K & \ding{51}  & Function  &  \ding{55} &  0   & No Limit  & 200  \\
    DevEval~[\citenum{li2024deveval}]   & 1  & \ding{55}  &  \ding{51}  & -- & 0.3K & \ding{51}  & File  &  \ding{55} &  164   & 2023.11-2024.02  & 1,825  \\
    \midrule
    \multicolumn{12}{l}{\textit{\textbf{The first category benchmarks}}} \\
    \midrule
    RepoQA~[\citenum{liu2024repoqa}] &    1   &  \ding{55}    &   \ding{55}   & 16K  &  --   &  \ding{55}   &   Function    &  \ding{55}   &  50     &   No Limit    &  500    \\ 
    L-Eval~[\citenum{an2023eval}] &    1   &  \ding{55}    &   \ding{55}   & 36.5K  &  31.5K   &  \ding{55}   &   Function    &  \ding{55}   &  0    &   No Limit    &  90    \\ 
    \rowcolor{blue!20} \method   & 8 & \ding{51} & \ding{51}  & 128K & 54.8K & \ding{51}    & File & \ding{51}   & 116  & 2024.06--2024.11   &  3,983  \\
    \bottomrule
    \end{tabular}%
        }
    \label{tab:benchmark comparision}%
\end{table*}%






























% Long-context language models (LCLMs) such as Gemini-1.5 \cite{team2024gemini} and GPT-4o \cite{achiam2023gpt} have support for context window length up to thousands of tokens. These LCLMs provide opportunities for long code generation and are evaluated on diverse long code generation benchmarks (\eg LongBench \cite{bai2023longbench} and Long Code Arena \cite{bogomolov2024long}). Different from generating one single code unit, long code generation needs LCLMs to process, understand, or even learn information from long-context dependencies and documentation in repositories. Long code understanding is the foundation of long code generation. Evaluating the long code understanding ability of LCLMs is inevitable for intelligent long code generation and even next-generation real-world software development. 
% \fang{The motivation of constructing LongCodeU needs improvement: the importance/necessity of long code understanding should not be limited to offering help for code generation (if so, further experiments to analysis the performance comparison between code generation and understanding is necessary). Suggestion: The ability of understanding long code context serves as a cornerstone for advanced applications in software engineering, providing more accurate and context-aware assistance, such as generating code, identifying bugs, suggesting optimizations, automating documentation, etc. However, xxx is under-explored.}
% \lilei{I think we can say that long-context LLMs demonstrate promising results on long-context benchmarks (RULER, L-EVAL etc.), setting a great foundation for aiding software engineering practices such as repo-level code generation. however, the evaluation of long-code U is under-explored, which is different from long context eval since the dependency between code snippets is more complex. Skip the discussion between code understanding and generation would be ok.}
% Long-context language models (LCLMs) such as Gemini-1.5 \cite{team2024gemini} and GPT-4o \cite{achiam2023gpt} have demonstrated promising results on long-context understanding benchmarks (\eg RULER \cite{hsieh2024ruler}, LongBench \cite{bai2023longbench}, etc.). This sets a great foundation for real-world software engineering practices, particularly in tasks like repository-level code generation, bug location, and long code summarization. However, the evaluation of long code understanding is under-explored, which is different from long-context evaluation since the dependency between source code is more complex. 




%引用
%  \verb|\citet| (cite in text)  \citet{Gusfield:97}.
 
%  \verb|\citep| (cite in parentheses)   \citep{Gusfield:97}.

%  \verb|\citealp| (alternative cite without parentheses) (e.g. \citealp{Gusfield:97}).

==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/2-LongCodeU_Benchmark.tex <==

\vspace{-2mm}

\section{\textbfmethod Benchmark}
\label{benchmark}





\begin{figure}[t]
\centering
\setlength{\belowcaptionskip}{-5mm}
\setlength{\abovecaptionskip}{0.1cm}
\includegraphics[width=\columnwidth]{latex/figure/workflow_4.pdf}
\caption{Four understanding aspects in \method.}
\label{figure: jzt}
\end{figure}


In this section, we first introduce long code understanding tasks (\textsection \ref{tasks}). Then, we describe the construction process of \method (\textsection \ref{benchmark construction}). Finally, we present the evaluation metrics (\textsection \ref{subsec:auto_eval}). 



\subsection{Tasks} \label{tasks}

In real-world software development, long code understanding is usually oriented towards code repositories. These repositories take functions as basic code units, establish relations among units to achieve complex applications, and introduce documentation to describe code-related information. LCLMs with good long code understanding abilities should be able to perceive and understand basic code units, relations among units, and associated code documentation, which is essentially required for dealing with downstream tasks such as repository-level code generation, issue resolving, and long code summarization. In this paper, we propose \method to comprehensively evaluate LCLMs' long code understanding ability from four aspects: code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long documentation understanding.
Four aspects of \method are shown in Figure \ref{figure: jzt}

%需要更复杂的符号描述
These long code understanding tasks share the following procedure: given an instruction, long code, and anchor input, LCLMs output the desired answer. The instruction briefly describes the request of each task. The anchor input is the detailed demand such as a code unit. In \method, instruction and anchor input are generally short, while long code is long containing 0$\sim$128K tokens. 





\subsubsection{Code Unit Perception}

Understanding long code, particularly in code repositories, requires identifying its numerous functions, as they form the foundational code unit for comprehending long code's overall functionality. 
In this paper, we treat a function as the code unit and introduce the code unit perception task to evaluate LCLMs' code unit identifying ability in long code. 
Concretely, this task requires LCLMs to identify all defined functions in long code and return their corresponding function names, where long code is composed of one or more code file contents collected from real-world repositories. 
This ability is the cornerstone for downstream tasks. 





\subsubsection{Intra-Code Unit Understanding}

Based on code unit perception, we further evaluate LCLMs' ability to understand the internal logic and semantics of code units. 

\paragraph{Code Unit Data Flow Analysis.}
In this section, we propose the code unit data flow analysis task that verifies whether LCLMs can understand the internal logic of code units by tracking data flow to a certain extent. Given a code unit in long code and a variable name in the code unit, LCLMs are required to figure out lines where the value of the given variable changes by tracing data flow. For example, after executing the line ``upper\_string += 2", the value of variable ``upper\_string" changes. The given code unit is randomly selected from long code and its position in long code is also random. Evaluating code unit understanding ability is significant for LCLMs to discover potential vulnerabilities, repair vulnerabilities, and optimize code.




\paragraph{Code Unit Semantic Analysis.}
In addition to analyzing the data flow of code units, we propose the code unit semantic analysis task to further verify LCLMs' intra-code unit understanding ability. 
The task asks LCLMs to return a code unit from the long code that satisfies the given description. The long code contains real-world code files, where all descriptions of code units are removed to prevent LCLMs from acquiring clues in them. 
This task requires LCLMs understand the semantics of code units and then return the desired code unit.



\subsubsection{Inter-Code Unit Relation Understanding}

In real-world long code, especially in code repositories, code units are non-standalone. Grasping code unit relations is essential for LCLMs to understand the complex functionality of long code, where code unit relations mainly containing dependency relations and semantic relations. The dependency relation indicates the calls among code units. The semantic relation focuses on the functional similarities of code units.



\paragraph{Dependency Relation Analysis.}
\textbf{(T1)}
Given a code unit, this task requires LCLMs to find code units that are invoked by the given unit from long code, where the long code covers one or multiple code files and is collected from the same repository with the given code unit. The dependency relation analysis ability can assist LCLMs correctly identifying other code units related to vulnerable units and determining vulnerability scopes in real-world applications.
\textbf{(T2)}
Considering that in real-world applications, apart from long code as LCLMs' input, developers usually use natural language requirements to interact with LCLMs. Thus, LCLMs also need to understand dependency relation between long code and requirements. Given a natural language description, this task requires LCLMs to find code units from the long code that are invoked for generating the desired code that satisfies the given description.
The ability can ensure that LCLMs sucessfully invoke existing code units in repository-level code generation and correctly integrate generated code into the current repository. 





\paragraph{Semantic Relation Extraction.}
Even if two code units have no dependency relationship, they might be semantically similar such as having similar implementation or logic. This section analyzes semantic relations of code units in long code. 
\textbf{(T1)} 
Given a code unit, this task asks LCLMs to extract semantically similar code units with the given unit from long code. Extracting semantic relations of units can effectively help LCLMs to improve software development efficiency by reusing similar code units when programming, and enhance software maintainability such as finding potentially similar vulnerabilities among semantically similar units.
\textbf{(T2)}
As described in dependency relation analysis (T2), understanding the semantical relations of code units and natural language requirements is more in line with practical development scenarios. For instance, in repository-level code generation, developers input a requirement to LCLMs. LCLMs can find semantically similar units with the given requirement from the current repository and then refer to these units to generate desired codes. 
In this task, LCLMs need to extract semantically similar code units to a given requirement, which challenges LCLMs to understand the semantics of units in long code and reason their semantic relations.


\subsubsection{Long Documentation Understanding}
In real-world software engineering, code documentation also plays a crucial role. It encompasses a diverse range of code-related information including descriptions of code units, usage patterns, architecture designs, and more. Consequently, it is essential not merely to verify the long code understanding ability, but also to analyze the long code documentation understanding ability of LCLMs. We introduce the long documentation understanding task. Given long documentation and a code unit name such as a function name contained in the documentation, this task requires LCLMs to extract the related information to the unit name. We ensure that the long documentation contains the related knowledge of the given unit name, aiming to effectively evaluate LCLMs. Analyzing long documentation is critical to verify the performance of LCLMs in real-world software development.




\begin{table}[t!]
  \centering
  \setlength{\abovecaptionskip}{0.1cm}
  \caption{Statistics of \method. \#Num means the number of examples in each task. \#C-File represents whether the output can be obtained by aggregating cross-file content. \#Avg-L is the average length of the output. \#Gran means the granularity of the output.}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lcc|ccc}
    \toprule
    \multirow{2}[4]{*}{Task} & \multicolumn{2}{c|}{Input}   & \multicolumn{3}{c}{Output} \\
\cmidrule{2-6}     & \multicolumn{1}{c}{\#Num} & \multicolumn{1}{c|}{Format} & \multicolumn{1}{c}{\#C-File} & \multicolumn{1}{c}{\#Avg-L} & \multicolumn{1}{c}{\#Gran} \\
    \midrule
    CU\_P     &  487 & Code      &  \ding{55} & 0.4K  & Name  \\
    CU\_SA    & 500 &  Code  & \ding{55}  & 0.2K & Function \\
    \midrule
    CU\_DFA      & 500   &  Code  & \ding{55}   & 0.03K & Line \\
    \midrule
    DRA\_T1     & 500   &  Code & \ding{51}  &  0.3K  & Function \\
    DRA\_T2    &500    & Code  & \ding{51}  & 0.3K  & Function \\
    SRE\_T1      & 500   &  Code  & \ding{51}  & 1.0K      & Function \\
    SRE\_T2   &  500  & Code & \ding{51}  & 1.1K  & Function \\
    \midrule
    LDU    & 500  &  Document  & \ding{55}  & 0.7K  & NL \\
    \bottomrule
    \end{tabular}%
     }
     \vspace{-0.4cm}
     \label{tab:Statistics of benchmark}%
\end{table}%







\vspace{-1mm}

\subsection{Benchmark Construction}  \label{benchmark construction}

The pipeline for constructing \method encompasses 6 stages as follows.

\noindent \textbf{Stage \ding{182}: Repository Selection.}
Referring to the TIOBE index \cite{Tiobe} for programming language popularity, the most popular language is Python. Thus, we conduct experiments on Python and will expand to other languages in the future. In Python source platforms, PyPI is a rich Python package index tool. We identify the top 10 popular programming topics in PyPI and obtain the top 50 packages with the most stars in each topic. We then select repositories following four criteria: open-source repositories, created after 2024-06, non-fork and non-malicious, and more than 50 stars. Finally, we crawl these repositories from GitHub and obtain 116 real-world repositories.

\noindent \textbf{Stage \ding{183}: Code Parse.}
We use \textit{tree-sitter}\footnote{https://tree-sitter.github.io/tree-sitter/} to design a code parser. This parser identifies code units defined in repositories, traces the definition of code units, and analyzes unit relations: First, it performs static analysis of each file in a repository and extracts unit names defined in it. Then, it executes unit symbol navigation, finding the definitions of all code units in the repository. Finally, it extracts unit names invoked in a code unit to grasp their dependency relations. Combining the three steps, the parser can traverse predefined code units within a repository and obtain intricate dependencies. To obtain semantic relations among units, we apply an advanced embedding model to encode code units, and use the cosine similarities of their representations to measure semantic relations. 



\noindent \textbf{Stage \ding{184}: Requirement Collection.}
We extract requirements contained in the signature of code units with \textit{tree-sitter} and invite two developers to check requirements. Not that it is enough to construct examples for T2-type tasks even if some code units do not contain requirements in repositories.  



\noindent \textbf{Stage \ding{185}: Documentation Annotation.}
We collect documentation from collected code repositories and select the documentation with standard: being easy to distinguish the related information of code units. Then we invite two developers to manually label 500 examples.


 
\noindent \textbf{Stage \ding{186}: Deduplication.}
For tasks whose input is code unit, we exclude trivial units (\eg empty or initialization functions). To ensure the quality of \method, we randomly select files from repositories as long codes, and ensure long codes of all examples in each task are non-repetitive.


\noindent \textbf{Stage \ding{187}: Benchmark Construction.}
Based on the above stages, we construct around 500 examples for each task supporting the maximum length of 128K tokens.
We make \method satisfy following goals: comprehensive tasks from practical applications, extra-long code context, real-world repositories, and reducing data contamination.




\subsection{Automatic Evaluation} \label{subsec:auto_eval}

We focus on evaluating the long code understanding ability required for LCLMs to complete downstream tasks. Tasks in \method commonly require LCLMs to retrieve dispersive snippets from long code and execute reasoning. Thus, we mainly adopt metrics used in retrieval tasks to measure LCLMs, including recall and precision.

For proper evaluation, we refine existing metrics according to the output granularity of tasks: 
\ding{182} \textit{Output with code lines} refers to the code unit data flow analysis task, which extracts several lines from long code. We first use exact match (\textbf{EM}) to measure each line in outputs. Then, we calculate recall and precision based on EM, acquiring \textbf{EM-R} and \textbf{EM-P} metrics.
\ding{183} \textit{Output with code unit names} is related to the code unit perception task. We first find the correct names in output and then calculate the longest common subsequence (LCS) of unit names between output and ground truth, since it not only reflects whether the unit name is correct but also indicates LCLMs' ability to perceive the position of units in long code. Then, we calculate recall and precision based on LCS, named \textbf{LCS-R} and \textbf{LCS-P}.
\ding{184} \textit{Output with code units} refers to code unit semantic analysis and inter-code unit relation understanding tasks. Code unit semantic analysis only returns one unit. We use \textbf{CodeBLEU} as its metric, where it is a popular metric to indicate the consistency of two code sequences. For inter-code unit relation understanding, it returns multiple code units. We first determine whether the name of each generated unit is in ground truth. Then, we calculate CodeBLEU of each unit if it exists in the ground truth. For the code unit whose name is not in the ground truth, its CodeBLEU value is set to 0. Based on CodeBLEU value of each unit, we finally calculate CodeBLEU-based recall and precision, dubbed \textbf{CB-R} and \textbf{CB-P}.
\ding{185} \textit{Output with descriptions} is related to the long documentation understanding task. Considering that documentation contains many text descriptions, we employ \textbf{BLEU} for evaluation, which is commonly used to measure the consistency between two sequences in the natural language process field.


These automatic evaluations can effectively measure LCLMs' long code understanding ability since the outputs of each task are deterministic and task' features are incorporated into these metrics. Figure \ref{figure: Reliable Evaluation Metrics} shows the automatic evaluation correlates well with human annotation, which further demonstrates the reliability of our automatic metrics.





==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/3-Experimental_Setup.tex <==
\section{Experimental Setup}






==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/4-Evaluation.tex <==
\begin{table*}[htbp]
  \centering
  \setlength{\abovecaptionskip}{0.1cm}
  \setlength{\belowcaptionskip}{-5mm}
  \caption{The performance of LCLMs on \method. 
  % \#Param means the parameter size of LCLMs. 
  We only report recall-based results (EM-R, LCS-R, and CB-R) due to page limitation. The precision-based results (EM-P, LCS-P, and CB-P) can be found in Appendix \ref{sec:appendix-rq2}.} 
    \label{tab: main results}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lcc|c|cc|cccc|c|c}
    \toprule
    \multirow{2}[2]{*}{} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{\#Param}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Context Size}}} & \multicolumn{9}{c}{\textbf{Task}}  \\
          &       &       & \multicolumn{1}{c|}{\textbf{CU\_P}} & \multicolumn{1}{c}{\textbf{CU\_SA}} & \multicolumn{1}{c|}{\textbf{CU\_DFA}} & \multicolumn{1}{c}{\textbf{DRA\_T1}} & \multicolumn{1}{c}{\textbf{DRA\_T2}} & \multicolumn{1}{c}{\textbf{SRE\_T1}} & \multicolumn{1}{c|}{\textbf{SRE\_T2}} & \multicolumn{1}{c|}{\textbf{LDU}}  & \multicolumn{1}{c|}{\textbf{\#Avg}}   \\
    \midrule
    \textit{Code Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}} \\
    Qwen2.5-Coder     & 7.6B & 128K  & \cellcolor{yellow!30}43.47 & \cellcolor{green!30}71.06 & \cellcolor{green!30}74.01 & \cellcolor{blue!25}30.38  & \cellcolor{blue!25}9.59 & \cellcolor{blue!25}24.34  & \cellcolor{blue!25}21.81   & \cellcolor{red!30}21.83   & 37.06 \\
    DeepSeek-Coder-V2     & 15.7B &  128K  & \cellcolor{yellow!30}38.67  & \cellcolor{green!30}65.21 & \cellcolor{green!30}48.42 & \cellcolor{blue!25}47.26 & \cellcolor{blue!25}22.92 &  \cellcolor{blue!25}24.61     & \cellcolor{blue!25}26.21 & \cellcolor{red!30}50.69     & 40.49 \\
    CodeLlama    &  33.7B  & 16K  & \cellcolor{yellow!30}68.57  & \cellcolor{green!30}62.41  &\cellcolor{green!30}79.87  & \cellcolor{blue!25}68.82  &\cellcolor{blue!25} 34.94 & \cellcolor{blue!25}44.48 &  \cellcolor{blue!25}36.34  &\cellcolor{red!30} 46.92  & 55.29 \\
    \midrule
    \textit{General Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}}  \\
    Phi-3.5     &  3.8B  &128K  & \cellcolor{yellow!30}39.92  & \cellcolor{green!30}46.75  & \cellcolor{green!30}49.52 &\cellcolor{blue!25}30.76  & \cellcolor{blue!25}9.66 & \cellcolor{blue!25}18.99  & \cellcolor{blue!25}14.48    & \cellcolor{red!30}34.14    & 30.53  \\
    Mistral-v0.3     &  7.3B  & 32K & \cellcolor{yellow!30}57.42  & \cellcolor{green!30}63.90 & \cellcolor{green!30}58.00  & \cellcolor{blue!25}46.66 & \cellcolor{blue!25}18.92 & \cellcolor{blue!25}33.91  & \cellcolor{blue!25}32.50 & \cellcolor{red!30}58.64    & 46.24 \\
    DeepSeek-V2.5     &  236B  &  128K   & \cellcolor{yellow!30}\textbf{70.58} & \cellcolor{green!30}82.11  & \cellcolor{green!30}77.47 & \cellcolor{blue!25}72.25 & \cellcolor{blue!25}\textbf{56.80}  & \cellcolor{blue!25}\textbf{49.08} & \cellcolor{blue!25}\textbf{47.42}  & \cellcolor{red!30}85.85    & \textbf{67.70} \\
\cmidrule{2-12}          & \multicolumn{11}{c}{\textit{Proprietary Source LCLMs}} \\
    Claude-3.5-Sonnet    & --  & 200K & \cellcolor{yellow!30}43.82 & \cellcolor{green!30}40.60 & \cellcolor{green!30}45.65 & \cellcolor{blue!25}29.37 & \cellcolor{blue!25}28.70 & \cellcolor{blue!25}26.55 & \cellcolor{blue!25}27.77 & \cellcolor{red!30}41.81    &35.53  \\
    Gemini-1.5-Flash     &  --  & 1000K & \cellcolor{yellow!30}58.45  & \cellcolor{green!30}83.46  & \cellcolor{green!30}80.37 & \cellcolor{blue!25}\textbf{72.51} & \cellcolor{blue!25}46.42 & \cellcolor{blue!25}39.84 & \cellcolor{blue!25}38.69  &\cellcolor{red!30} 81.43    &61.39 \\
    GPT-4o     & --  & 128K  & \cellcolor{yellow!30}56.42 & \cellcolor{green!30}\textbf{86.76}  & \cellcolor{green!30}\textbf{87.87} & \cellcolor{blue!25}71.58 &\cellcolor{blue!25} 48.88 & \cellcolor{blue!25}44.45  & \cellcolor{blue!25}43.14  & \cellcolor{red!30}\textbf{87.54}    & \textbf{65.83} \\
    \bottomrule
    \end{tabular}%
     }
\end{table*}%



\vspace{-2mm}

\section{Experiment Setups} \label{sec: evaluation}


In this section, we aim to answer the following research questions through a series of experiments. 


\noindent\textbf{RQ1. How is the long code understanding ability of LCLMs?} We evaluate LCLMs' long code understanding ability on \method in \S\ref{Long Code Understanding Capability}.

\noindent\textbf{RQ2. What is performance of LCLMs across long code lengths?} We explore the performance of LCLMs on long code with different lengths. \S\ref{Performance across Long Code Lengths} demonstrates LCLMs' performance comparison across long code lengths. 


\noindent\textbf{RQ3. How do developers select models in real-world application scenarios?} Based on the experimental results, we summarize the empirical lessons we learned, aiming to help developers select suitable LCLMs ~(\S\ref{subsec:downstream_task}).



\subsection{Base LCLMs}
We evaluate 9 advanced LCLMs on \method, which contain 6 general models (\ie GPT-4o \cite{GPT-4o}, Claude-3.5-Sonnet \cite{claude-3.5}, Gemini-1.5-Flash \cite{team2024gemini}, DeepSeek-V2.5 \cite{bai2023longbench}, Mistral-v0.3 \cite{jiang2023mistral}, and Phi-3.5 \cite{abdin2024phi} ) and 3 code models (\ie DeepSeek-Coder-V2 \cite{bai2023longbench},  Qwen2.5-Coder \cite{hui2024qwen2}, CodeLlama \cite{roziere2023code}). DeepSeek-R1 and GPT-o3-mini are newly released LCLMs, but their availability through invoking API is unstable or limited to usage frequency. We can not present their performance now and will evaluate them in the future.



\subsection{Experimental Setup}
We use greedy search for all experiments. We evaluate LCLMs within their maximum context window length. In the semantic relation extraction task, we use an advanced embedding model stella\_en\_400M\_v5 to encode code units and natural language requirements with the 1,024 dimension version, and select the top five similar code units by calculating the cosine similarities of their embeddings. Constrained by computing resources, we evaluate DeepSeek-V2.5 by invoking API\footnote{https://api-docs.deepseek.com/api/deepseek-api} provided by DeepSeek. 
Although the context length of DeepSeek-V2.5 achieves 128K tokens, the API provided by DeepSeek only supports up to 60K tokens. Thus, we analyze DeepSeek-V2.5 on long codes with 0$\sim$64K tokens.
















\section{Results and Analysis} \label{sec: evaluation}



% % Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table*}[htbp]
%   \centering
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcc|c|cc|cccc|c}
%     \toprule
%     \multirow{2}[2]{*}{} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{\#Param}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Context Size}}} & \multicolumn{8}{c}{\textbf{Task}} \\
%           &       &       & \multicolumn{1}{c|}{\textbf{CU\_P}} & \multicolumn{1}{c}{\textbf{CU\_SA}} & \multicolumn{1}{c|}{\textbf{CU\_DFA}} & \multicolumn{1}{c}{\textbf{DRA\_T1}} & \multicolumn{1}{c}{\textbf{DRA\_T2}} & \multicolumn{1}{c}{\textbf{SRE\_T1}} & \multicolumn{1}{c|}{\textbf{SRE\_T2}} & \multicolumn{1}{c}{\textbf{LDU}} \\
%     \midrule
%     \textit{Code Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}} \\
%     Qwen2.5-Coder     & 7.6B & 128K  & 43.47 & 71.06 & 74.01 & 30.38  & 9.59 & 24.34  & 21.81   & 21.83 \\
%     DeepSeek-Coder-V2     & 15.7B &  128K  & 38.67  & 65.21 & 48.42 & 47.26 & 22.92 &  24.61     & 26.21 & 50.69 \\
%     CodeLlama    &  33.7B  & 16K  & 68.57  & 62.41  & 79.87  & 68.82  & 34.94 & 44.48 &  36.34  & 46.92 \\
%     \midrule
%     \textit{General Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}}  \\
%     Phi-3.5     &  3.8B  &128K  & 39.92  & 46.75  & 49.52 &30.76  & 9.66 & 18.99  & 14.48    & 34.14 \\
%     Mistral-v0.3     &  7.3B  & 32K & 57.42  & 63.90 & 58.00  & 46.66 & 18.92 & 33.91  & 32.50 & 58.64 \\
%     DeepSeek-V2.5     &  236B  &  128K   & \textbf{70.58} & 82.11  & 77.47 & 72.25 & \textbf{56.80}  & \textbf{49.08} & \textbf{47.42}  & 85.85 \\
% \cmidrule{2-11}          & \multicolumn{10}{c}{\textit{Proprietary Source LCLMs}} \\
%     Claude-3-Haiku    & --  & 200K & 16.26 & 12.15 & 8.00 & 3.25 & 3.91 & 3.15 & 2.77 & 10.73 \\
%     Claude-3-5-Sonnet    & --  & 200K & 43.82 & 40.60 & 45.65 & 29.37 & 28.70 & 26.55 & 27.77 & 41.81 \\
%     Gemini-1.5-Flash     &  --  & 1000K & 58.45  & 83.46  & 80.37 & \textbf{72.51} & 46.42 & 39.84 & 38.69  & 81.43 \\
%     GPT-4o     & --  & 128K  & 56.42 & \textbf{86.76}  & \textbf{87.87} & 71.58 & 48.88 & 44.45  & 43.14  & \textbf{87.54}  \\
%     \bottomrule
%     \end{tabular}%
%      }
%    \caption{The performance of LCLMs on \method. \#Param means the parameter size of LCLMs. Constrained by space limitations, we only report recall-based results (\ie EM-R, LCS-R, and CB-R) for related tasks. The precision-based results (\ie EM-P, LCS-P, and CB-P) are presented in \textbf{AppendiX}.} 
%     \label{tab: main results}
% \end{table*}%










\begin{figure*}[t]
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-5mm}
% \setlength{\abovecaptionskip}{-1mm}
\includegraphics[width=\linewidth]{latex/figure/results_41.pdf}
\caption{Performance comparison across tasks and long code lengths on \method (grey blocks indicate unavailable configurations). The rate of performance degradation exhibits task-specific and model-specific patterns. }
\label{Figure: heat map}
\end{figure*}



\subsection{Long Code Understanding Capability} \label{Long Code Understanding Capability}

Table~\ref{tab: main results} presents the performance of LCLMs on \method.  
%which only contains recall-based results for related tasks constrained by space limitations. The precision-based results are shown in \textbf{Appendix}. 
For LCLMs with a context length of less than 128K tokens, we only evaluate them within their supporting maximum lengths. 


\paragraph{Comparison across LCLMs.}
%same scale 尺寸的代码模型比通用模型表现好; 在开源模型中， 开源模型deepseekv2.5表现最好，并且在多个任务上超越4o等闭园模型，可能因为参数量和训练方式 数据等。在闭园模型中，4o表现最好；claude 有待提升，尤其是3-haiku（意义）。模型使用建议：有资源 没资源 效果要求高低
We observe significant performance gaps among LCLMs. 
For similar-scale models, the performance of code LCLMs is better than the counterpart of general models on most tasks. For example, Qwen2.5-Coder outperforms Phi-3.5 24.31\% on intra-code unit understanding (the second-aspect task) in terms of CodeBLEU, and DeepSeek-Coder-V2 achieves 11.75\% average improvements on inter-code unit relation understanding (the third-aspect task) in CB-R. Among open-source models, DeepSeek-V2.5 performs the best, which is related to its large number of parameters. In proprietary source models, GPT-4o achieves the best performance, while Claude-3.5-Sonnet is not satisfactory. %, especially for Claude-3-Haiku. 



\paragraph{Comparison across Tasks.}
%对于四种类型的任务，模型在xx和xxx表现较好，其次是xxx,最差是xx. 这是合理的，因为对于实际的代码库，大模型感知代码单元是基础，在感知基础上理解单元功能，解析单元之间的关系，从而理解长代码。
%在关系分析任务中，相似关系提取的表现低于依赖关系提取，这是因为？
%没有模型在所有任务上表现都好。对于尺寸相似的通用和代码模型，，代码模型在感知任务上高于通用模型，然而在文档理解任务上，通用模型比代码模型表现好。
In the four aspects, LCLMs perform the best in code unit perception and long documentation understanding, and achieve moderate results in intra-unit code understanding. Inter-code unit relation understanding is the most challenging. 
Their performances are reasonable. Because it's a fundamental ability for LCLMs to understand code documentation and perceive code units. Based on this, LCLMs understand intra-unit code and then analyze inter-code unit relations, thereby comprehending long code.
When observing the third-aspect task (\ie inter-code unit relation understanding) closely, it can be seen that the performance of dependency relation analysis is lower than that of semantic relation extraction. 
We also find that no LCLM outperforms others on all tasks. For instance, in terms of scale-similar code models and general models, the former outperforms the latter in code unit perception, while code models perform worse than general models in long documentation understanding.







\subsection{Performance across Long Code Lengths} \label{Performance across Long Code Lengths}
%为了解决rq2，我们在具有不同代码长度的样本上进行实验，以探究大模型真正支持的上下文长度在代码理解任务上。图xx展示了模型在具有不同代码长度的样本上的结果。
%我们可以看到代码长度和模型表现呈现负相关关系。具体而言，在代码长度为0-32k的表现几乎满意，当代码长度超过32k后，所有模型性能急剧下降。例如。
%在很多人任务上，大多数模型在64-128k间性能接近为0.
%%在不同代码长度上，模型性能变化的斜率不同。
To address RQ2, we classify examples into five buckets according to the long code length, including 0$\sim$8K, 8$\sim$16K, 16$\sim$32K, 32$\sim$64K, and 64$\sim$128K on each task. We conduct experiments on these classes to investigate the true context ability supported by LCLMs in long code understanding. Figure \ref{Figure: heat map} and Appendix \ref{sec:appendix-rq2} shows the results of LCLMs across long code lengths. % on \method. 

Our experimental results reveal key limitations in current LCLMs’ capabilities for long code understanding. 
We can also observe a negative correlation between the long code length and the performance of LCLMs. 
LCLMs' performance drops dramatically when the long code length is greater than 32K tokens, falling well short of their claimed 128K$\sim$1M context windows.
Besides, when the long code contains 64$\sim$128K tokens, the performance of LCLMs is near to 10 or even close to 0 on some tasks such as dependency relation analysis and semantic relation extraction.
In addition, the degradation slopes of performances vary by task. For example, there is a large slope in long documentation understanding, which means that LCLMs are suitable for processing relatively short documentation. The slope on code unit understanding including code unit data flow analysis and code unit semantic analysis tasks is relatively small.  LCLMs fail to model code context effectively in their claimed context windows.

% LCLMs exhibit consistent performance degradation with increased long code length. LCLMs achieve near-satisfying results in 0$\sim$32K. However, \textbf{LCLMs' performance drops dramatically when the long code length is greater than 32K, falling well short of their claimed context windows with 128K tokens or more.} For example, GPT-4o's performance drops from 73.34 at 0$\sim$8K to 29.62 at 64$\sim$128K. In addition, some LCLMs, such as DeepSeek-Coder-V2 and Phi-3.5, perform less than 10 or even almost 0 at 64$\sim$128K on some tasks. For instance, Phi-3.5 only achieves 3.99 on the semantic relation extraction task. These performances underscore the significant room for improving long code understanding.
% II) Performance degradation rates vary by task. We observe steeper performance degradation in Long Documentation Understanding. Results of DeepSeek-V2 and Qwen 2.5 drop from 82.76 and 54.63 to 8.18 and 8.27. Note that LCLMs perform steadily on Context Dependency Analysis across 0$\sim$128K, although some models achieve approximately 50\% and others only perform around 10\%.




% \subsection{Long Code Understanding vs. Downstream Tasks}
% \label{subsec:downstream_task}
% \method aims to evaluate LCLMs' long code understanding ability by ask models to identify code units, understand code units, analyze the relstions of code units, and understand long code documentation. These capabilities are essential for real-world downstream tasks. In this section, we investigate how the long code understanding ability of LCLMs affect the performance of downstream tasks as described in RQ3. 

% Figure \textbf{xxx} demonstrates the relations between the performance of long code understanding and the results of downstream tasks on the same LCLM.
%由于指标不同，结果归一化。曲线，横坐标下游任务的表现0-1，纵坐标不同模型在同一个下游任务上的表现0-1，不同曲线为不同下游任务，曲线上节点为不同模型 

% swebench: https://www.all-hands.dev/blog/evaluation-of-llms-as-coding-agents-on-swe-bench-at-30x-speed
% evocodebench: jia li
% code translation: tse yanlin wang 








% 模型选择建议
\subsection{Empirical Lessons.} \label{subsec:downstream_task}
% 根据模型的表现，我们给大家提供一些模型选择建议。
% 不同模型（性能退化程度，没有一个模型在任务和长度的可比规模下始终优于其他模型）
% 资源 任务需求侧重点
Based on the above experiments, we summarize the empirical lessons we learned as:
%当对代码单元感知有需求时。当常见的长代码不超过16K时，选择较小的模型就可以达到不错的效果；对于较长文档选择qw或者闭园4o gimi
\ding{182} The small-size LCLMs such as Qwen2.5-Coder can satisfy developers' need for code unit perception and understanding if long code length is less than 16K. Otherwise, we suggest choosing larger-size models. 
%对于长文档理解有需求的，尤其是文档超过32k,建议使用xx
\ding{183} For understanding long code documentation with more than 32K tokens, it is recommended to use GPT-4o and Gemini-1.5-Flash. Otherwise, Mistral-v0.3 and DeepSeek-Coder-V2 can achieve satisfying performances.
%当对下游任务对代码单元理解要求较高时（如代码检索任务），并且长代码较长时，开源建议选择2.5 ，闭园选gm 4o
% \ding{184} When developers have high requirements for code unit understanding, we do not suggest using Claude-3.5-Sonnet and Phi-3.5.
%对于关系较高的任务，比如生成、漏洞，建议选择最强的开源和闭园模型。当长代码超过64k时，即使较强模型，能力很弱，因此可能会限制在这类下游任务上的效果。比如xx模型在python-jave翻译上能力几乎为0。
\ding{184} 
For tasks with high requirements for understanding inter-code unit relations, we suggest selecting the most powerful LCLMs that developers can access. Because when long code length exceeds 64K which is common in repository-level tasks, strong LCLMs also achieve weak perfrmances. These poor performances explain why powerful LCLMs perform unsatisfactorily in repository-level downstream tasks. For example, GPT-4o only achieves 4.00\% Success@1 on repository-level code translation benchmark-RepoTransBench \cite{DBLP:journals/corr/abs-2412-17744}.









% If developers have sufficient computing resources, we suggest to use DeepSeek-V2.5, otherwish it is recommended to use GPT-4o or DeepSeek-Coder-V2.



==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/5-Analysis.tex <==

\section{Discussion}


\subsection{Case Study}

We analyze the outputs of LCLMs, particularly GPT-4o, on the inter-code unit relation understanding task. Appendix \ref{sec:appendix-case} presents two notable examples. GPT-4o often extracts code units that are structurally similar or share overlapping tokens but have distinct or even opposite functionalities. This highlights the need to enhance models' ability to distinguish confusing code units.




\subsection{Code Understanding or Memorization?}

We collect a small number of early-released code repositories from GitHub that LCLMs have potentially encountered during LCLMs training, aiming to analyze the dependency degree of LCLMs on memorization and long code understanding ability. Concretely, we enter only an instruction and anchor input to models, withholding the long code context, and assess their performance. We select tasks where models can work normally even without long code context, such as code unit semantic analysis and dependency relation analysis (T2). As shown in Figure~\ref{figure: memory}, the memorization performance (w/o context) is much lower than the results with long code context, even though models might have met these contexts when training. The $\delta$ score (the results with context minus the performance without context in yellow) relieves the memory phenomenon \cite{yu2023kola} and also reveals the significant importance for measuring LCLMs' long code understanding ability. 




\subsection{Reliable Evaluation Metrics?}

Reliable evaluation metrics are essential for assessing long code understanding. We measure the consistency between our metrics and human evaluation by selecting 20 GPT-4o outputs on each task and inviting two advanced developers to manually evaluate them. Using Kendall-Tau $\tau$ \cite{kendall1938new}, we found that the average $\tau$ value is at least 0.75 across all tasks, with the minimum value exceeding 0.7 (Figure \ref{figure: Reliable Evaluation Metrics}). This demonstrates a strong correlation between our metrics and human evaluation, confirming the reliability of our metrics. 







==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/6-Related_Works.tex <==
\section{Related Works} \label{related works}
\paragraph{Benchmarks on Long Code Understanding.} 

Existing studies can be mainly categorized into two types. 
The first category predominantly explores the long code understanding ability required in downstream applications like the needle-in-a-haystack task, but they face significant limitations. RepoQA \cite{liu2024repoqa} is a pioneer introduced needle function retrieval task. However, the single task is insufficient to evaluate the complex long code understanding ability. L-Eval \cite{an2023eval}, a widely-used benchmark, has limitations as well. It constructs artificial "long code" by concatenating independent code snippets, ignoring context dependency in real-world source code. 
These limitations highlight the need for a more comprehensive and reliable benchmarking approach for evaluating LCLMs' long code understanding ability. 
The second category includes research like LCArea \cite{bogomolov2024long}. They verify LCLMs' long code understanding ability by measuring their performance on downstream tasks such as LongBench \cite{bai2023longbench}, SWE-bench \cite{jimenez2023swe}, and EvoCodeBench \cite{li2024evocodebench}. Although they provide an intuitive way to assess LCLMs, it suffers from a significant drawback. The performance of downstream tasks is confounded by multiple factors, and these works do not decouple the long code understanding ability independently, which 
is orthogonal to our objective-evaluating LCLMs' capacity to understand and reason about real-world, dependency-rich, long code.



\paragraph{Long Context Language Models.}

Recent studies have explored diverse ways to extend large language models' context window size. The direct way is to fine-tune models on long sequences \cite{wu2021recursively}, but they are often effort-costing.
Some approaches involve additional fine-tuning for a longer context \cite{xiong2023effective, chen2023clex, chen2023extending, chen2023fortify, peng2023yarn}. They down-scale the input position indices to match the original context window size of models with several training steps. 
There are also some training-free studies, which use window attention to clip the long sequences \cite{han2023lm, ding2023longnet, xiao2023efficient}. 
Concurrently, a series of approaches modify the relative distance to extend the extrapolation length \cite{zhang2024hirope, jin2024llm}. In this paper, we construct a comprehensive benchmark to evaluate LCLMs' long code understanding ability.  


==> htrxbsmvndgfvqccwdpptrfnmykfctds/latex/7-Conclusion.tex <==
\vspace{-1mm}

\section{Conclusion}

In this paper, we propose a comprehensive long code understanding benchmark \method. It introduces four aspects (8 tasks) to evaluate LCLMs’ long code understanding ability required for practical applications, including code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long code documentation understanding. Our experimental results reveal key limitations in current LCLMs’ capabilities for long code understanding. 
When the long code length contains more than 32K tokens, 
the performance of LCLMs drops dramatically, falling far short of their claimed 128K$\sim$1M context windows. 
We hope our findings can provide valuable insights for optimizing LCLMs and driving advancements in software engineering.







\section*{Limitations}

This paper proposes a benchmark - \method to evaluate the long code understanding ability of long context language models from four aspects which are essential capabilities required for LCLMs to complete real-world downstream tasks. 
Based on \method, we evaluate 9 popular LCLMs and analyze their strengths and shortcomings. We think that DevEval has three limitations.


\ding{182} \method is a monolingual benchmark (\ie requirements in English and code in Python) and ignores other languages. In practice, LLMs require understanding requirements in different natural languages (\eg Chinese, Spanish) and generating programs in various programming languages (\eg Java, C). Thus, we plan to build a multilingual
\method in future work.

\ding{183} Most recently, there are a few newly released LCLMs such as DeepSeek-R1 and OpenAI o3-mini-high. Constrained by the availability or stabilization of API, we do not provide the performance of these newly released models. In the future, we will evaluate their long code understanding abilities on \method.

\ding{184} In our experiments, we only consider the long code with 0$\sim$128K tokens, although some LCLMs have supported longer context windows, \eg Claude-3-5-Sonnet with 200K context size and even Gemini-1.5-Flash with 1000K context size. We will continue to update and evolve our benchmark, in order to support \method to measure LCLMs on longer codes.



==> latex/1-Introduction.tex <==
\section{Introduction}
\label{Introduction}


\begin{figure}[t]
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-5mm}
\includegraphics[width=\columnwidth]{latex/figure/Introduction_example.pdf}
\caption{Examples of a synthetic long code with independent functions and a real-world long code with non-standalone functions. Dependencies are highlighted.}
\label{figure: benchmark comprison}
% \vspace{-0.4cm}
\end{figure}



Recent advances in long-context language models (LCLMs) like Gemini-1.5 \cite{team2024gemini} and GPT-4o \cite{GPT-4o}, which support context windows exceeding hundreds of thousands of tokens, offer unprecedented potential for real-world software engineering applications. These models promise transformative improvements in related downstream tasks, such as repository-level code generation \cite{zhang2024codeagent, bi2024iterative}, real-world GitHub issues resolution\cite{jimenez2023swe}, and long code summarization \cite{dhulshette2025hierarchical}. However, progress in this critical area remains hampered by a fundamental limitation: \textbf{the lack of rigorous evaluation frameworks for long code understanding}—a capability essential for real-world software development tools that require accurate code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long code documentation understanding in code repositories.








Current benchmarks generally fall into two categories, which face five fundamental limitations that hinder comprehensive evaluation of LCLMs' long code understanding capabilities.  
The first category includes studies such as RepoQA \cite{liu2024repoqa}, whose task design has insufficient diversity like only focusing on needle function search. While these evaluations are useful, \ding{182} \textbf{they do not capture the real-world full range of code understanding capabilities} needed for practical coding scenarios. Additionally, benchmarks like L-Eval \citet{an2023eval} further compound these limitations by using synthetic ``long code'' through a simple joining of independent code snippets. \ding{183} This approach \textbf{overlooks the natural dependencies between code segments}, as shown in Figure~\ref{figure: benchmark comprison}. 
\ding{184} These studies also face issues with \textbf{data contamination}. They neither enforce temporal constraints on code release dates nor address potential model pre-exposure through evaluating on previously published datasets. \ding{185} Their maximum supported context length of 36.5K tokens also \textbf{falls far short of stress-testing the claimed 128K-1M context windows of modern LCLMs}.
The second category includes benchmarks like Long Code Arena \cite{bogomolov2024long}, LongBench \cite{bai2023longbench}, SWE-bench \cite{jimenez2023swe}, and DevEval \cite{li2024deveval}, which evaluate long-context understanding based on performance in downstream tasks. 
\ding{186} However, these benchmarks \textbf{entangle code understanding with other task-specific challenges} like code generation and bug fixing.
This makes it hard to determine whether performance limitations are due to a lack of code understanding or other factors.


To address these limitations, we propose \method, a benchmark designed to isolate and comprehensively evaluate LCLMs' capacity to understand and reason about real-world, dependency-rich, long code contexts. Our benchmark offers the following key features:
\begin{itemize}[topsep=0pt,noitemsep] 
\item[$\bullet$] \textbf{Comprehensive Tasks stem from Practical Applications.} We evaluate LCLMs from four aspects (8 tasks) to evaluate the LCLMs' long code understanding capability required for practical applications, including code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long documentation understanding.


\item[$\bullet$] \textbf{Extra-long Code Context.} Each task contains around 500 gathered long codes. The lengths of examples change in 0$\sim$8K, 8$\sim$16K, 16$\sim$32K, 32$\sim$64K, and 64$\sim$128K following the normal distribution, which far exceeds the maximum length of 36.5K supported by existing benchmarks \cite{an2023eval}.


\item[$\bullet$] \textbf{Real-world Repository.} The benchmark is collected from real-world code repositories. Long code consists of one or more real code file contents, instead of being composed of multiple independent code units like current benchmarks \cite{liu2024repoqa}. 


\item[$\bullet$] \textbf{Reducing Data Contamination.} We collect up-to-date code repositories that are created after 2024-06 from GitHub\footnote{https://github.com/}, which are later than most prevailing LCLMs' cut-off dates thus reducing the risk of data contamination.

\end{itemize}


We evaluate 9 popular LCLMs, which contain 6 general models (\ie GPT-4o \cite{GPT-4o}, Claude-3.5-Sonnet \cite{claude-3.5}, Gemini-1.5-Flash \cite{team2024gemini}, DeepSeek-V2.5 \cite{bai2023longbench}, Mistral-v0.3 \cite{jiang2023mistral}, and Phi-3.5 \cite{abdin2024phi} ) and 3 code models (\ie DeepSeek-Coder-V2 \cite{bai2023longbench},  Qwen2.5-Coder \cite{hui2024qwen2}, CodeLlama \cite{roziere2023code}) on \method. 
The experimental results reveal key limitations in current LCLMs' capabilities for long code understanding. Especially, \textbf{LCLMs’ performance drops dramatically when the long code length is greater than 32K, falling far short of their claimed context windows such as 128K-1M tokens}. 
In the four aspects, \textbf{inter-code unit relation understanding is the most challenging for LCLMs.}
Our findings provide valuable insights for optimizing LCLMs and driving advancements in software engineering.



\begin{table*}[htbp]
  \centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-5mm}
\caption{The comparison between existing benchmarks and \method. \#Num is the abbreviation of number. \#Div Tasks refers to diverse tasks. \#High Disp represents high dispersion.  \#Max-L and \#Avg-L mean the maximum length and the average length of long code. \#Trunk-L means whether each example has the length label. \#Doc refers to documentation related to repositories. \#Task represents the number of tasks (\ie examples).}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|c|c}
    \toprule
    \multirow{2}[2]{*}{Benchmark} & \multicolumn{3}{c|}{Comprehensive Code Tasks}              & \multicolumn{3}{c|}{Extra-long Data} & \multicolumn{3}{c|}{Real-world Repository} & \multicolumn{1}{c|}{Reduce Data Leaking} & \multicolumn{1}{c}{Data Scale} \\
          & \multicolumn{1}{c}{\#Num} &  \multicolumn{1}{c}{\#Div Tasks}  & \multicolumn{1}{c|}{\#High Disp} & \multicolumn{1}{c}{\#Max-L} & \multicolumn{1}{c}{\#Avg-L} & \multicolumn{1}{c|}{\#Length-L} & \multicolumn{1}{c}{Code} & \multicolumn{1}{c}{\#Doc}  & \multicolumn{1}{c|}{\#Num} & \multicolumn{1}{c|}{Data Time}  & \multicolumn{1}{c}{\#Task} \\
    \midrule
    \multicolumn{12}{l}{\textit{\textbf{The second category benchmarks (Only some benchmarks are listed)}}} \\
    \midrule
    LongBench~[\citenum{bai2023longbench}]    &  2 &  \ding{55} &  \ding{55}  &  --  & 0.4K &  \ding{55}  &  Function &  \ding{55} &  -- &  2023.02--2023.08     &  1,000  \\
    LC-Arena~[\citenum{bogomolov2024long}]   &  6 &  \ding{55} &  \ding{55}  & -- & -- & \ding{55}   & File  & \ding{55}  & 62  &  2023.01--2024.05  & --   \\
    LONGPROC~[\citenum{ye2025longproc}]   & 1  & \ding{55}  &  \ding{51}  & -- & 2K & \ding{51}  & Function  &  \ding{55} &  0   & No Limit  & 200  \\
    DevEval~[\citenum{li2024deveval}]   & 1  & \ding{55}  &  \ding{51}  & -- & 0.3K & \ding{51}  & File  &  \ding{55} &  164   & 2023.11-2024.02  & 1,825  \\
    \midrule
    \multicolumn{12}{l}{\textit{\textbf{The first category benchmarks}}} \\
    \midrule
    RepoQA~[\citenum{liu2024repoqa}] &    1   &  \ding{55}    &   \ding{55}   & 16K  &  --   &  \ding{55}   &   Function    &  \ding{55}   &  50     &   No Limit    &  500    \\ 
    L-Eval~[\citenum{an2023eval}] &    1   &  \ding{55}    &   \ding{55}   & 36.5K  &  31.5K   &  \ding{55}   &   Function    &  \ding{55}   &  0    &   No Limit    &  90    \\ 
    \rowcolor{blue!20} \method   & 8 & \ding{51} & \ding{51}  & 128K & 54.8K & \ding{51}    & File & \ding{51}   & 116  & 2024.06--2024.11   &  3,983  \\
    \bottomrule
    \end{tabular}%
        }
    \label{tab:benchmark comparision}%
\end{table*}%






























% Long-context language models (LCLMs) such as Gemini-1.5 \cite{team2024gemini} and GPT-4o \cite{achiam2023gpt} have support for context window length up to thousands of tokens. These LCLMs provide opportunities for long code generation and are evaluated on diverse long code generation benchmarks (\eg LongBench \cite{bai2023longbench} and Long Code Arena \cite{bogomolov2024long}). Different from generating one single code unit, long code generation needs LCLMs to process, understand, or even learn information from long-context dependencies and documentation in repositories. Long code understanding is the foundation of long code generation. Evaluating the long code understanding ability of LCLMs is inevitable for intelligent long code generation and even next-generation real-world software development. 
% \fang{The motivation of constructing LongCodeU needs improvement: the importance/necessity of long code understanding should not be limited to offering help for code generation (if so, further experiments to analysis the performance comparison between code generation and understanding is necessary). Suggestion: The ability of understanding long code context serves as a cornerstone for advanced applications in software engineering, providing more accurate and context-aware assistance, such as generating code, identifying bugs, suggesting optimizations, automating documentation, etc. However, xxx is under-explored.}
% \lilei{I think we can say that long-context LLMs demonstrate promising results on long-context benchmarks (RULER, L-EVAL etc.), setting a great foundation for aiding software engineering practices such as repo-level code generation. however, the evaluation of long-code U is under-explored, which is different from long context eval since the dependency between code snippets is more complex. Skip the discussion between code understanding and generation would be ok.}
% Long-context language models (LCLMs) such as Gemini-1.5 \cite{team2024gemini} and GPT-4o \cite{achiam2023gpt} have demonstrated promising results on long-context understanding benchmarks (\eg RULER \cite{hsieh2024ruler}, LongBench \cite{bai2023longbench}, etc.). This sets a great foundation for real-world software engineering practices, particularly in tasks like repository-level code generation, bug location, and long code summarization. However, the evaluation of long code understanding is under-explored, which is different from long-context evaluation since the dependency between source code is more complex. 




%引用
%  \verb|\citet| (cite in text)  \citet{Gusfield:97}.
 
%  \verb|\citep| (cite in parentheses)   \citep{Gusfield:97}.

%  \verb|\citealp| (alternative cite without parentheses) (e.g. \citealp{Gusfield:97}).

==> latex/2-LongCodeU_Benchmark.tex <==

\vspace{-2mm}

\section{\textbfmethod Benchmark}
\label{benchmark}





\begin{figure}[t]
\centering
\setlength{\belowcaptionskip}{-5mm}
\setlength{\abovecaptionskip}{0.1cm}
\includegraphics[width=\columnwidth]{latex/figure/workflow_4.pdf}
\caption{Four understanding aspects in \method.}
\label{figure: jzt}
\end{figure}


In this section, we first introduce long code understanding tasks (\textsection \ref{tasks}). Then, we describe the construction process of \method (\textsection \ref{benchmark construction}). Finally, we present the evaluation metrics (\textsection \ref{subsec:auto_eval}). 



\subsection{Tasks} \label{tasks}

In real-world software development, long code understanding is usually oriented towards code repositories. These repositories take functions as basic code units, establish relations among units to achieve complex applications, and introduce documentation to describe code-related information. LCLMs with good long code understanding abilities should be able to perceive and understand basic code units, relations among units, and associated code documentation, which is essentially required for dealing with downstream tasks such as repository-level code generation, issue resolving, and long code summarization. In this paper, we propose \method to comprehensively evaluate LCLMs' long code understanding ability from four aspects: code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long documentation understanding.
Four aspects of \method are shown in Figure \ref{figure: jzt}

%需要更复杂的符号描述
These long code understanding tasks share the following procedure: given an instruction, long code, and anchor input, LCLMs output the desired answer. The instruction briefly describes the request of each task. The anchor input is the detailed demand such as a code unit. In \method, instruction and anchor input are generally short, while long code is long containing 0$\sim$128K tokens. 





\subsubsection{Code Unit Perception}

Understanding long code, particularly in code repositories, requires identifying its numerous functions, as they form the foundational code unit for comprehending long code's overall functionality. 
In this paper, we treat a function as the code unit and introduce the code unit perception task to evaluate LCLMs' code unit identifying ability in long code. 
Concretely, this task requires LCLMs to identify all defined functions in long code and return their corresponding function names, where long code is composed of one or more code file contents collected from real-world repositories. 
This ability is the cornerstone for downstream tasks. 





\subsubsection{Intra-Code Unit Understanding}

Based on code unit perception, we further evaluate LCLMs' ability to understand the internal logic and semantics of code units. 

\paragraph{Code Unit Data Flow Analysis.}
In this section, we propose the code unit data flow analysis task that verifies whether LCLMs can understand the internal logic of code units by tracking data flow to a certain extent. Given a code unit in long code and a variable name in the code unit, LCLMs are required to figure out lines where the value of the given variable changes by tracing data flow. For example, after executing the line ``upper\_string += 2", the value of variable ``upper\_string" changes. The given code unit is randomly selected from long code and its position in long code is also random. Evaluating code unit understanding ability is significant for LCLMs to discover potential vulnerabilities, repair vulnerabilities, and optimize code.




\paragraph{Code Unit Semantic Analysis.}
In addition to analyzing the data flow of code units, we propose the code unit semantic analysis task to further verify LCLMs' intra-code unit understanding ability. 
The task asks LCLMs to return a code unit from the long code that satisfies the given description. The long code contains real-world code files, where all descriptions of code units are removed to prevent LCLMs from acquiring clues in them. 
This task requires LCLMs understand the semantics of code units and then return the desired code unit.



\subsubsection{Inter-Code Unit Relation Understanding}

In real-world long code, especially in code repositories, code units are non-standalone. Grasping code unit relations is essential for LCLMs to understand the complex functionality of long code, where code unit relations mainly containing dependency relations and semantic relations. The dependency relation indicates the calls among code units. The semantic relation focuses on the functional similarities of code units.



\paragraph{Dependency Relation Analysis.}
\textbf{(T1)}
Given a code unit, this task requires LCLMs to find code units that are invoked by the given unit from long code, where the long code covers one or multiple code files and is collected from the same repository with the given code unit. The dependency relation analysis ability can assist LCLMs correctly identifying other code units related to vulnerable units and determining vulnerability scopes in real-world applications.
\textbf{(T2)}
Considering that in real-world applications, apart from long code as LCLMs' input, developers usually use natural language requirements to interact with LCLMs. Thus, LCLMs also need to understand dependency relation between long code and requirements. Given a natural language description, this task requires LCLMs to find code units from the long code that are invoked for generating the desired code that satisfies the given description.
The ability can ensure that LCLMs sucessfully invoke existing code units in repository-level code generation and correctly integrate generated code into the current repository. 





\paragraph{Semantic Relation Extraction.}
Even if two code units have no dependency relationship, they might be semantically similar such as having similar implementation or logic. This section analyzes semantic relations of code units in long code. 
\textbf{(T1)} 
Given a code unit, this task asks LCLMs to extract semantically similar code units with the given unit from long code. Extracting semantic relations of units can effectively help LCLMs to improve software development efficiency by reusing similar code units when programming, and enhance software maintainability such as finding potentially similar vulnerabilities among semantically similar units.
\textbf{(T2)}
As described in dependency relation analysis (T2), understanding the semantical relations of code units and natural language requirements is more in line with practical development scenarios. For instance, in repository-level code generation, developers input a requirement to LCLMs. LCLMs can find semantically similar units with the given requirement from the current repository and then refer to these units to generate desired codes. 
In this task, LCLMs need to extract semantically similar code units to a given requirement, which challenges LCLMs to understand the semantics of units in long code and reason their semantic relations.


\subsubsection{Long Documentation Understanding}
In real-world software engineering, code documentation also plays a crucial role. It encompasses a diverse range of code-related information including descriptions of code units, usage patterns, architecture designs, and more. Consequently, it is essential not merely to verify the long code understanding ability, but also to analyze the long code documentation understanding ability of LCLMs. We introduce the long documentation understanding task. Given long documentation and a code unit name such as a function name contained in the documentation, this task requires LCLMs to extract the related information to the unit name. We ensure that the long documentation contains the related knowledge of the given unit name, aiming to effectively evaluate LCLMs. Analyzing long documentation is critical to verify the performance of LCLMs in real-world software development.




\begin{table}[t!]
  \centering
  \setlength{\abovecaptionskip}{0.1cm}
  \caption{Statistics of \method. \#Num means the number of examples in each task. \#C-File represents whether the output can be obtained by aggregating cross-file content. \#Avg-L is the average length of the output. \#Gran means the granularity of the output.}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lcc|ccc}
    \toprule
    \multirow{2}[4]{*}{Task} & \multicolumn{2}{c|}{Input}   & \multicolumn{3}{c}{Output} \\
\cmidrule{2-6}     & \multicolumn{1}{c}{\#Num} & \multicolumn{1}{c|}{Format} & \multicolumn{1}{c}{\#C-File} & \multicolumn{1}{c}{\#Avg-L} & \multicolumn{1}{c}{\#Gran} \\
    \midrule
    CU\_P     &  487 & Code      &  \ding{55} & 0.4K  & Name  \\
    CU\_SA    & 500 &  Code  & \ding{55}  & 0.2K & Function \\
    \midrule
    CU\_DFA      & 500   &  Code  & \ding{55}   & 0.03K & Line \\
    \midrule
    DRA\_T1     & 500   &  Code & \ding{51}  &  0.3K  & Function \\
    DRA\_T2    &500    & Code  & \ding{51}  & 0.3K  & Function \\
    SRE\_T1      & 500   &  Code  & \ding{51}  & 1.0K      & Function \\
    SRE\_T2   &  500  & Code & \ding{51}  & 1.1K  & Function \\
    \midrule
    LDU    & 500  &  Document  & \ding{55}  & 0.7K  & NL \\
    \bottomrule
    \end{tabular}%
     }
     \vspace{-0.4cm}
     \label{tab:Statistics of benchmark}%
\end{table}%







\vspace{-1mm}

\subsection{Benchmark Construction}  \label{benchmark construction}

The pipeline for constructing \method encompasses 6 stages as follows.

\noindent \textbf{Stage \ding{182}: Repository Selection.}
Referring to the TIOBE index \cite{Tiobe} for programming language popularity, the most popular language is Python. Thus, we conduct experiments on Python and will expand to other languages in the future. In Python source platforms, PyPI is a rich Python package index tool. We identify the top 10 popular programming topics in PyPI and obtain the top 50 packages with the most stars in each topic. We then select repositories following four criteria: open-source repositories, created after 2024-06, non-fork and non-malicious, and more than 50 stars. Finally, we crawl these repositories from GitHub and obtain 116 real-world repositories.

\noindent \textbf{Stage \ding{183}: Code Parse.}
We use \textit{tree-sitter}\footnote{https://tree-sitter.github.io/tree-sitter/} to design a code parser. This parser identifies code units defined in repositories, traces the definition of code units, and analyzes unit relations: First, it performs static analysis of each file in a repository and extracts unit names defined in it. Then, it executes unit symbol navigation, finding the definitions of all code units in the repository. Finally, it extracts unit names invoked in a code unit to grasp their dependency relations. Combining the three steps, the parser can traverse predefined code units within a repository and obtain intricate dependencies. To obtain semantic relations among units, we apply an advanced embedding model to encode code units, and use the cosine similarities of their representations to measure semantic relations. 



\noindent \textbf{Stage \ding{184}: Requirement Collection.}
We extract requirements contained in the signature of code units with \textit{tree-sitter} and invite two developers to check requirements. Not that it is enough to construct examples for T2-type tasks even if some code units do not contain requirements in repositories.  



\noindent \textbf{Stage \ding{185}: Documentation Annotation.}
We collect documentation from collected code repositories and select the documentation with standard: being easy to distinguish the related information of code units. Then we invite two developers to manually label 500 examples.


 
\noindent \textbf{Stage \ding{186}: Deduplication.}
For tasks whose input is code unit, we exclude trivial units (\eg empty or initialization functions). To ensure the quality of \method, we randomly select files from repositories as long codes, and ensure long codes of all examples in each task are non-repetitive.


\noindent \textbf{Stage \ding{187}: Benchmark Construction.}
Based on the above stages, we construct around 500 examples for each task supporting the maximum length of 128K tokens.
We make \method satisfy following goals: comprehensive tasks from practical applications, extra-long code context, real-world repositories, and reducing data contamination.




\subsection{Automatic Evaluation} \label{subsec:auto_eval}

We focus on evaluating the long code understanding ability required for LCLMs to complete downstream tasks. Tasks in \method commonly require LCLMs to retrieve dispersive snippets from long code and execute reasoning. Thus, we mainly adopt metrics used in retrieval tasks to measure LCLMs, including recall and precision.

For proper evaluation, we refine existing metrics according to the output granularity of tasks: 
\ding{182} \textit{Output with code lines} refers to the code unit data flow analysis task, which extracts several lines from long code. We first use exact match (\textbf{EM}) to measure each line in outputs. Then, we calculate recall and precision based on EM, acquiring \textbf{EM-R} and \textbf{EM-P} metrics.
\ding{183} \textit{Output with code unit names} is related to the code unit perception task. We first find the correct names in output and then calculate the longest common subsequence (LCS) of unit names between output and ground truth, since it not only reflects whether the unit name is correct but also indicates LCLMs' ability to perceive the position of units in long code. Then, we calculate recall and precision based on LCS, named \textbf{LCS-R} and \textbf{LCS-P}.
\ding{184} \textit{Output with code units} refers to code unit semantic analysis and inter-code unit relation understanding tasks. Code unit semantic analysis only returns one unit. We use \textbf{CodeBLEU} as its metric, where it is a popular metric to indicate the consistency of two code sequences. For inter-code unit relation understanding, it returns multiple code units. We first determine whether the name of each generated unit is in ground truth. Then, we calculate CodeBLEU of each unit if it exists in the ground truth. For the code unit whose name is not in the ground truth, its CodeBLEU value is set to 0. Based on CodeBLEU value of each unit, we finally calculate CodeBLEU-based recall and precision, dubbed \textbf{CB-R} and \textbf{CB-P}.
\ding{185} \textit{Output with descriptions} is related to the long documentation understanding task. Considering that documentation contains many text descriptions, we employ \textbf{BLEU} for evaluation, which is commonly used to measure the consistency between two sequences in the natural language process field.


These automatic evaluations can effectively measure LCLMs' long code understanding ability since the outputs of each task are deterministic and task' features are incorporated into these metrics. Figure \ref{figure: Reliable Evaluation Metrics} shows the automatic evaluation correlates well with human annotation, which further demonstrates the reliability of our automatic metrics.





==> latex/3-Experimental_Setup.tex <==
\section{Experimental Setup}






==> latex/4-Evaluation.tex <==
\begin{table*}[htbp]
  \centering
  \setlength{\abovecaptionskip}{0.1cm}
  \setlength{\belowcaptionskip}{-5mm}
  \caption{The performance of LCLMs on \method. 
  % \#Param means the parameter size of LCLMs. 
  We only report recall-based results (EM-R, LCS-R, and CB-R) due to page limitation. The precision-based results (EM-P, LCS-P, and CB-P) can be found in Appendix \ref{sec:appendix-rq2}.} 
    \label{tab: main results}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lcc|c|cc|cccc|c|c}
    \toprule
    \multirow{2}[2]{*}{} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{\#Param}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Context Size}}} & \multicolumn{9}{c}{\textbf{Task}}  \\
          &       &       & \multicolumn{1}{c|}{\textbf{CU\_P}} & \multicolumn{1}{c}{\textbf{CU\_SA}} & \multicolumn{1}{c|}{\textbf{CU\_DFA}} & \multicolumn{1}{c}{\textbf{DRA\_T1}} & \multicolumn{1}{c}{\textbf{DRA\_T2}} & \multicolumn{1}{c}{\textbf{SRE\_T1}} & \multicolumn{1}{c|}{\textbf{SRE\_T2}} & \multicolumn{1}{c|}{\textbf{LDU}}  & \multicolumn{1}{c|}{\textbf{\#Avg}}   \\
    \midrule
    \textit{Code Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}} \\
    Qwen2.5-Coder     & 7.6B & 128K  & \cellcolor{yellow!30}43.47 & \cellcolor{green!30}71.06 & \cellcolor{green!30}74.01 & \cellcolor{blue!25}30.38  & \cellcolor{blue!25}9.59 & \cellcolor{blue!25}24.34  & \cellcolor{blue!25}21.81   & \cellcolor{red!30}21.83   & 37.06 \\
    DeepSeek-Coder-V2     & 15.7B &  128K  & \cellcolor{yellow!30}38.67  & \cellcolor{green!30}65.21 & \cellcolor{green!30}48.42 & \cellcolor{blue!25}47.26 & \cellcolor{blue!25}22.92 &  \cellcolor{blue!25}24.61     & \cellcolor{blue!25}26.21 & \cellcolor{red!30}50.69     & 40.49 \\
    CodeLlama    &  33.7B  & 16K  & \cellcolor{yellow!30}68.57  & \cellcolor{green!30}62.41  &\cellcolor{green!30}79.87  & \cellcolor{blue!25}68.82  &\cellcolor{blue!25} 34.94 & \cellcolor{blue!25}44.48 &  \cellcolor{blue!25}36.34  &\cellcolor{red!30} 46.92  & 55.29 \\
    \midrule
    \textit{General Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}}  \\
    Phi-3.5     &  3.8B  &128K  & \cellcolor{yellow!30}39.92  & \cellcolor{green!30}46.75  & \cellcolor{green!30}49.52 &\cellcolor{blue!25}30.76  & \cellcolor{blue!25}9.66 & \cellcolor{blue!25}18.99  & \cellcolor{blue!25}14.48    & \cellcolor{red!30}34.14    & 30.53  \\
    Mistral-v0.3     &  7.3B  & 32K & \cellcolor{yellow!30}57.42  & \cellcolor{green!30}63.90 & \cellcolor{green!30}58.00  & \cellcolor{blue!25}46.66 & \cellcolor{blue!25}18.92 & \cellcolor{blue!25}33.91  & \cellcolor{blue!25}32.50 & \cellcolor{red!30}58.64    & 46.24 \\
    DeepSeek-V2.5     &  236B  &  128K   & \cellcolor{yellow!30}\textbf{70.58} & \cellcolor{green!30}82.11  & \cellcolor{green!30}77.47 & \cellcolor{blue!25}72.25 & \cellcolor{blue!25}\textbf{56.80}  & \cellcolor{blue!25}\textbf{49.08} & \cellcolor{blue!25}\textbf{47.42}  & \cellcolor{red!30}85.85    & \textbf{67.70} \\
\cmidrule{2-12}          & \multicolumn{11}{c}{\textit{Proprietary Source LCLMs}} \\
    Claude-3.5-Sonnet    & --  & 200K & \cellcolor{yellow!30}43.82 & \cellcolor{green!30}40.60 & \cellcolor{green!30}45.65 & \cellcolor{blue!25}29.37 & \cellcolor{blue!25}28.70 & \cellcolor{blue!25}26.55 & \cellcolor{blue!25}27.77 & \cellcolor{red!30}41.81    &35.53  \\
    Gemini-1.5-Flash     &  --  & 1000K & \cellcolor{yellow!30}58.45  & \cellcolor{green!30}83.46  & \cellcolor{green!30}80.37 & \cellcolor{blue!25}\textbf{72.51} & \cellcolor{blue!25}46.42 & \cellcolor{blue!25}39.84 & \cellcolor{blue!25}38.69  &\cellcolor{red!30} 81.43    &61.39 \\
    GPT-4o     & --  & 128K  & \cellcolor{yellow!30}56.42 & \cellcolor{green!30}\textbf{86.76}  & \cellcolor{green!30}\textbf{87.87} & \cellcolor{blue!25}71.58 &\cellcolor{blue!25} 48.88 & \cellcolor{blue!25}44.45  & \cellcolor{blue!25}43.14  & \cellcolor{red!30}\textbf{87.54}    & \textbf{65.83} \\
    \bottomrule
    \end{tabular}%
     }
\end{table*}%



\vspace{-2mm}

\section{Experiment Setups} \label{sec: evaluation}


In this section, we aim to answer the following research questions through a series of experiments. 


\noindent\textbf{RQ1. How is the long code understanding ability of LCLMs?} We evaluate LCLMs' long code understanding ability on \method in \S\ref{Long Code Understanding Capability}.

\noindent\textbf{RQ2. What is performance of LCLMs across long code lengths?} We explore the performance of LCLMs on long code with different lengths. \S\ref{Performance across Long Code Lengths} demonstrates LCLMs' performance comparison across long code lengths. 


\noindent\textbf{RQ3. How do developers select models in real-world application scenarios?} Based on the experimental results, we summarize the empirical lessons we learned, aiming to help developers select suitable LCLMs ~(\S\ref{subsec:downstream_task}).



\subsection{Base LCLMs}
We evaluate 9 advanced LCLMs on \method, which contain 6 general models (\ie GPT-4o \cite{GPT-4o}, Claude-3.5-Sonnet \cite{claude-3.5}, Gemini-1.5-Flash \cite{team2024gemini}, DeepSeek-V2.5 \cite{bai2023longbench}, Mistral-v0.3 \cite{jiang2023mistral}, and Phi-3.5 \cite{abdin2024phi} ) and 3 code models (\ie DeepSeek-Coder-V2 \cite{bai2023longbench},  Qwen2.5-Coder \cite{hui2024qwen2}, CodeLlama \cite{roziere2023code}). DeepSeek-R1 and GPT-o3-mini are newly released LCLMs, but their availability through invoking API is unstable or limited to usage frequency. We can not present their performance now and will evaluate them in the future.



\subsection{Experimental Setup}
We use greedy search for all experiments. We evaluate LCLMs within their maximum context window length. In the semantic relation extraction task, we use an advanced embedding model stella\_en\_400M\_v5 to encode code units and natural language requirements with the 1,024 dimension version, and select the top five similar code units by calculating the cosine similarities of their embeddings. Constrained by computing resources, we evaluate DeepSeek-V2.5 by invoking API\footnote{https://api-docs.deepseek.com/api/deepseek-api} provided by DeepSeek. 
Although the context length of DeepSeek-V2.5 achieves 128K tokens, the API provided by DeepSeek only supports up to 60K tokens. Thus, we analyze DeepSeek-V2.5 on long codes with 0$\sim$64K tokens.
















\section{Results and Analysis} \label{sec: evaluation}



% % Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table*}[htbp]
%   \centering
%     \resizebox{1\linewidth}{!}{
%     \begin{tabular}{lcc|c|cc|cccc|c}
%     \toprule
%     \multirow{2}[2]{*}{} & \multicolumn{1}{c}{\multirow{2}[2]{*}{\textbf{\#Param}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Context Size}}} & \multicolumn{8}{c}{\textbf{Task}} \\
%           &       &       & \multicolumn{1}{c|}{\textbf{CU\_P}} & \multicolumn{1}{c}{\textbf{CU\_SA}} & \multicolumn{1}{c|}{\textbf{CU\_DFA}} & \multicolumn{1}{c}{\textbf{DRA\_T1}} & \multicolumn{1}{c}{\textbf{DRA\_T2}} & \multicolumn{1}{c}{\textbf{SRE\_T1}} & \multicolumn{1}{c|}{\textbf{SRE\_T2}} & \multicolumn{1}{c}{\textbf{LDU}} \\
%     \midrule
%     \textit{Code Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}} \\
%     Qwen2.5-Coder     & 7.6B & 128K  & 43.47 & 71.06 & 74.01 & 30.38  & 9.59 & 24.34  & 21.81   & 21.83 \\
%     DeepSeek-Coder-V2     & 15.7B &  128K  & 38.67  & 65.21 & 48.42 & 47.26 & 22.92 &  24.61     & 26.21 & 50.69 \\
%     CodeLlama    &  33.7B  & 16K  & 68.57  & 62.41  & 79.87  & 68.82  & 34.94 & 44.48 &  36.34  & 46.92 \\
%     \midrule
%     \textit{General Models} & \multicolumn{10}{c}{\textit{Open-Source LCLMs}}  \\
%     Phi-3.5     &  3.8B  &128K  & 39.92  & 46.75  & 49.52 &30.76  & 9.66 & 18.99  & 14.48    & 34.14 \\
%     Mistral-v0.3     &  7.3B  & 32K & 57.42  & 63.90 & 58.00  & 46.66 & 18.92 & 33.91  & 32.50 & 58.64 \\
%     DeepSeek-V2.5     &  236B  &  128K   & \textbf{70.58} & 82.11  & 77.47 & 72.25 & \textbf{56.80}  & \textbf{49.08} & \textbf{47.42}  & 85.85 \\
% \cmidrule{2-11}          & \multicolumn{10}{c}{\textit{Proprietary Source LCLMs}} \\
%     Claude-3-Haiku    & --  & 200K & 16.26 & 12.15 & 8.00 & 3.25 & 3.91 & 3.15 & 2.77 & 10.73 \\
%     Claude-3-5-Sonnet    & --  & 200K & 43.82 & 40.60 & 45.65 & 29.37 & 28.70 & 26.55 & 27.77 & 41.81 \\
%     Gemini-1.5-Flash     &  --  & 1000K & 58.45  & 83.46  & 80.37 & \textbf{72.51} & 46.42 & 39.84 & 38.69  & 81.43 \\
%     GPT-4o     & --  & 128K  & 56.42 & \textbf{86.76}  & \textbf{87.87} & 71.58 & 48.88 & 44.45  & 43.14  & \textbf{87.54}  \\
%     \bottomrule
%     \end{tabular}%
%      }
%    \caption{The performance of LCLMs on \method. \#Param means the parameter size of LCLMs. Constrained by space limitations, we only report recall-based results (\ie EM-R, LCS-R, and CB-R) for related tasks. The precision-based results (\ie EM-P, LCS-P, and CB-P) are presented in \textbf{AppendiX}.} 
%     \label{tab: main results}
% \end{table*}%










\begin{figure*}[t]
\centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-5mm}
% \setlength{\abovecaptionskip}{-1mm}
\includegraphics[width=\linewidth]{latex/figure/results_41.pdf}
\caption{Performance comparison across tasks and long code lengths on \method (grey blocks indicate unavailable configurations). The rate of performance degradation exhibits task-specific and model-specific patterns. }
\label{Figure: heat map}
\end{figure*}



\subsection{Long Code Understanding Capability} \label{Long Code Understanding Capability}

Table~\ref{tab: main results} presents the performance of LCLMs on \method.  
%which only contains recall-based results for related tasks constrained by space limitations. The precision-based results are shown in \textbf{Appendix}. 
For LCLMs with a context length of less than 128K tokens, we only evaluate them within their supporting maximum lengths. 


\paragraph{Comparison across LCLMs.}
%same scale 尺寸的代码模型比通用模型表现好; 在开源模型中， 开源模型deepseekv2.5表现最好，并且在多个任务上超越4o等闭园模型，可能因为参数量和训练方式 数据等。在闭园模型中，4o表现最好；claude 有待提升，尤其是3-haiku（意义）。模型使用建议：有资源 没资源 效果要求高低
We observe significant performance gaps among LCLMs. 
For similar-scale models, the performance of code LCLMs is better than the counterpart of general models on most tasks. For example, Qwen2.5-Coder outperforms Phi-3.5 24.31\% on intra-code unit understanding (the second-aspect task) in terms of CodeBLEU, and DeepSeek-Coder-V2 achieves 11.75\% average improvements on inter-code unit relation understanding (the third-aspect task) in CB-R. Among open-source models, DeepSeek-V2.5 performs the best, which is related to its large number of parameters. In proprietary source models, GPT-4o achieves the best performance, while Claude-3.5-Sonnet is not satisfactory. %, especially for Claude-3-Haiku. 



\paragraph{Comparison across Tasks.}
%对于四种类型的任务，模型在xx和xxx表现较好，其次是xxx,最差是xx. 这是合理的，因为对于实际的代码库，大模型感知代码单元是基础，在感知基础上理解单元功能，解析单元之间的关系，从而理解长代码。
%在关系分析任务中，相似关系提取的表现低于依赖关系提取，这是因为？
%没有模型在所有任务上表现都好。对于尺寸相似的通用和代码模型，，代码模型在感知任务上高于通用模型，然而在文档理解任务上，通用模型比代码模型表现好。
In the four aspects, LCLMs perform the best in code unit perception and long documentation understanding, and achieve moderate results in intra-unit code understanding. Inter-code unit relation understanding is the most challenging. 
Their performances are reasonable. Because it's a fundamental ability for LCLMs to understand code documentation and perceive code units. Based on this, LCLMs understand intra-unit code and then analyze inter-code unit relations, thereby comprehending long code.
When observing the third-aspect task (\ie inter-code unit relation understanding) closely, it can be seen that the performance of dependency relation analysis is lower than that of semantic relation extraction. 
We also find that no LCLM outperforms others on all tasks. For instance, in terms of scale-similar code models and general models, the former outperforms the latter in code unit perception, while code models perform worse than general models in long documentation understanding.







\subsection{Performance across Long Code Lengths} \label{Performance across Long Code Lengths}
%为了解决rq2，我们在具有不同代码长度的样本上进行实验，以探究大模型真正支持的上下文长度在代码理解任务上。图xx展示了模型在具有不同代码长度的样本上的结果。
%我们可以看到代码长度和模型表现呈现负相关关系。具体而言，在代码长度为0-32k的表现几乎满意，当代码长度超过32k后，所有模型性能急剧下降。例如。
%在很多人任务上，大多数模型在64-128k间性能接近为0.
%%在不同代码长度上，模型性能变化的斜率不同。
To address RQ2, we classify examples into five buckets according to the long code length, including 0$\sim$8K, 8$\sim$16K, 16$\sim$32K, 32$\sim$64K, and 64$\sim$128K on each task. We conduct experiments on these classes to investigate the true context ability supported by LCLMs in long code understanding. Figure \ref{Figure: heat map} and Appendix \ref{sec:appendix-rq2} shows the results of LCLMs across long code lengths. % on \method. 

Our experimental results reveal key limitations in current LCLMs’ capabilities for long code understanding. 
We can also observe a negative correlation between the long code length and the performance of LCLMs. 
LCLMs' performance drops dramatically when the long code length is greater than 32K tokens, falling well short of their claimed 128K$\sim$1M context windows.
Besides, when the long code contains 64$\sim$128K tokens, the performance of LCLMs is near to 10 or even close to 0 on some tasks such as dependency relation analysis and semantic relation extraction.
In addition, the degradation slopes of performances vary by task. For example, there is a large slope in long documentation understanding, which means that LCLMs are suitable for processing relatively short documentation. The slope on code unit understanding including code unit data flow analysis and code unit semantic analysis tasks is relatively small.  LCLMs fail to model code context effectively in their claimed context windows.

% LCLMs exhibit consistent performance degradation with increased long code length. LCLMs achieve near-satisfying results in 0$\sim$32K. However, \textbf{LCLMs' performance drops dramatically when the long code length is greater than 32K, falling well short of their claimed context windows with 128K tokens or more.} For example, GPT-4o's performance drops from 73.34 at 0$\sim$8K to 29.62 at 64$\sim$128K. In addition, some LCLMs, such as DeepSeek-Coder-V2 and Phi-3.5, perform less than 10 or even almost 0 at 64$\sim$128K on some tasks. For instance, Phi-3.5 only achieves 3.99 on the semantic relation extraction task. These performances underscore the significant room for improving long code understanding.
% II) Performance degradation rates vary by task. We observe steeper performance degradation in Long Documentation Understanding. Results of DeepSeek-V2 and Qwen 2.5 drop from 82.76 and 54.63 to 8.18 and 8.27. Note that LCLMs perform steadily on Context Dependency Analysis across 0$\sim$128K, although some models achieve approximately 50\% and others only perform around 10\%.




% \subsection{Long Code Understanding vs. Downstream Tasks}
% \label{subsec:downstream_task}
% \method aims to evaluate LCLMs' long code understanding ability by ask models to identify code units, understand code units, analyze the relstions of code units, and understand long code documentation. These capabilities are essential for real-world downstream tasks. In this section, we investigate how the long code understanding ability of LCLMs affect the performance of downstream tasks as described in RQ3. 

% Figure \textbf{xxx} demonstrates the relations between the performance of long code understanding and the results of downstream tasks on the same LCLM.
%由于指标不同，结果归一化。曲线，横坐标下游任务的表现0-1，纵坐标不同模型在同一个下游任务上的表现0-1，不同曲线为不同下游任务，曲线上节点为不同模型 

% swebench: https://www.all-hands.dev/blog/evaluation-of-llms-as-coding-agents-on-swe-bench-at-30x-speed
% evocodebench: jia li
% code translation: tse yanlin wang 








% 模型选择建议
\subsection{Empirical Lessons.} \label{subsec:downstream_task}
% 根据模型的表现，我们给大家提供一些模型选择建议。
% 不同模型（性能退化程度，没有一个模型在任务和长度的可比规模下始终优于其他模型）
% 资源 任务需求侧重点
Based on the above experiments, we summarize the empirical lessons we learned as:
%当对代码单元感知有需求时。当常见的长代码不超过16K时，选择较小的模型就可以达到不错的效果；对于较长文档选择qw或者闭园4o gimi
\ding{182} The small-size LCLMs such as Qwen2.5-Coder can satisfy developers' need for code unit perception and understanding if long code length is less than 16K. Otherwise, we suggest choosing larger-size models. 
%对于长文档理解有需求的，尤其是文档超过32k,建议使用xx
\ding{183} For understanding long code documentation with more than 32K tokens, it is recommended to use GPT-4o and Gemini-1.5-Flash. Otherwise, Mistral-v0.3 and DeepSeek-Coder-V2 can achieve satisfying performances.
%当对下游任务对代码单元理解要求较高时（如代码检索任务），并且长代码较长时，开源建议选择2.5 ，闭园选gm 4o
% \ding{184} When developers have high requirements for code unit understanding, we do not suggest using Claude-3.5-Sonnet and Phi-3.5.
%对于关系较高的任务，比如生成、漏洞，建议选择最强的开源和闭园模型。当长代码超过64k时，即使较强模型，能力很弱，因此可能会限制在这类下游任务上的效果。比如xx模型在python-jave翻译上能力几乎为0。
\ding{184} 
For tasks with high requirements for understanding inter-code unit relations, we suggest selecting the most powerful LCLMs that developers can access. Because when long code length exceeds 64K which is common in repository-level tasks, strong LCLMs also achieve weak perfrmances. These poor performances explain why powerful LCLMs perform unsatisfactorily in repository-level downstream tasks. For example, GPT-4o only achieves 4.00\% Success@1 on repository-level code translation benchmark-RepoTransBench \cite{DBLP:journals/corr/abs-2412-17744}.









% If developers have sufficient computing resources, we suggest to use DeepSeek-V2.5, otherwish it is recommended to use GPT-4o or DeepSeek-Coder-V2.



==> latex/5-Analysis.tex <==

\section{Discussion}


\subsection{Case Study}

We analyze the outputs of LCLMs, particularly GPT-4o, on the inter-code unit relation understanding task. Appendix \ref{sec:appendix-case} presents two notable examples. GPT-4o often extracts code units that are structurally similar or share overlapping tokens but have distinct or even opposite functionalities. This highlights the need to enhance models' ability to distinguish confusing code units.




\subsection{Code Understanding or Memorization?}

We collect a small number of early-released code repositories from GitHub that LCLMs have potentially encountered during LCLMs training, aiming to analyze the dependency degree of LCLMs on memorization and long code understanding ability. Concretely, we enter only an instruction and anchor input to models, withholding the long code context, and assess their performance. We select tasks where models can work normally even without long code context, such as code unit semantic analysis and dependency relation analysis (T2). As shown in Figure~\ref{figure: memory}, the memorization performance (w/o context) is much lower than the results with long code context, even though models might have met these contexts when training. The $\delta$ score (the results with context minus the performance without context in yellow) relieves the memory phenomenon \cite{yu2023kola} and also reveals the significant importance for measuring LCLMs' long code understanding ability. 




\subsection{Reliable Evaluation Metrics?}

Reliable evaluation metrics are essential for assessing long code understanding. We measure the consistency between our metrics and human evaluation by selecting 20 GPT-4o outputs on each task and inviting two advanced developers to manually evaluate them. Using Kendall-Tau $\tau$ \cite{kendall1938new}, we found that the average $\tau$ value is at least 0.75 across all tasks, with the minimum value exceeding 0.7 (Figure \ref{figure: Reliable Evaluation Metrics}). This demonstrates a strong correlation between our metrics and human evaluation, confirming the reliability of our metrics. 







==> latex/6-Related_Works.tex <==
\section{Related Works} \label{related works}
\paragraph{Benchmarks on Long Code Understanding.} 

Existing studies can be mainly categorized into two types. 
The first category predominantly explores the long code understanding ability required in downstream applications like the needle-in-a-haystack task, but they face significant limitations. RepoQA \cite{liu2024repoqa} is a pioneer introduced needle function retrieval task. However, the single task is insufficient to evaluate the complex long code understanding ability. L-Eval \cite{an2023eval}, a widely-used benchmark, has limitations as well. It constructs artificial "long code" by concatenating independent code snippets, ignoring context dependency in real-world source code. 
These limitations highlight the need for a more comprehensive and reliable benchmarking approach for evaluating LCLMs' long code understanding ability. 
The second category includes research like LCArea \cite{bogomolov2024long}. They verify LCLMs' long code understanding ability by measuring their performance on downstream tasks such as LongBench \cite{bai2023longbench}, SWE-bench \cite{jimenez2023swe}, and EvoCodeBench \cite{li2024evocodebench}. Although they provide an intuitive way to assess LCLMs, it suffers from a significant drawback. The performance of downstream tasks is confounded by multiple factors, and these works do not decouple the long code understanding ability independently, which 
is orthogonal to our objective-evaluating LCLMs' capacity to understand and reason about real-world, dependency-rich, long code.



\paragraph{Long Context Language Models.}

Recent studies have explored diverse ways to extend large language models' context window size. The direct way is to fine-tune models on long sequences \cite{wu2021recursively}, but they are often effort-costing.
Some approaches involve additional fine-tuning for a longer context \cite{xiong2023effective, chen2023clex, chen2023extending, chen2023fortify, peng2023yarn}. They down-scale the input position indices to match the original context window size of models with several training steps. 
There are also some training-free studies, which use window attention to clip the long sequences \cite{han2023lm, ding2023longnet, xiao2023efficient}. 
Concurrently, a series of approaches modify the relative distance to extend the extrapolation length \cite{zhang2024hirope, jin2024llm}. In this paper, we construct a comprehensive benchmark to evaluate LCLMs' long code understanding ability.  


==> latex/7-Conclusion.tex <==
\vspace{-1mm}

\section{Conclusion}

In this paper, we propose a comprehensive long code understanding benchmark \method. It introduces four aspects (8 tasks) to evaluate LCLMs’ long code understanding ability required for practical applications, including code unit perception, intra-code unit understanding, inter-code unit relation understanding, and long code documentation understanding. Our experimental results reveal key limitations in current LCLMs’ capabilities for long code understanding. 
When the long code length contains more than 32K tokens, 
the performance of LCLMs drops dramatically, falling far short of their claimed 128K$\sim$1M context windows. 
We hope our findings can provide valuable insights for optimizing LCLMs and driving advancements in software engineering.







\section*{Limitations}

This paper proposes a benchmark - \method to evaluate the long code understanding ability of long context language models from four aspects which are essential capabilities required for LCLMs to complete real-world downstream tasks. 
Based on \method, we evaluate 9 popular LCLMs and analyze their strengths and shortcomings. We think that DevEval has three limitations.


\ding{182} \method is a monolingual benchmark (\ie requirements in English and code in Python) and ignores other languages. In practice, LLMs require understanding requirements in different natural languages (\eg Chinese, Spanish) and generating programs in various programming languages (\eg Java, C). Thus, we plan to build a multilingual
\method in future work.

\ding{183} Most recently, there are a few newly released LCLMs such as DeepSeek-R1 and OpenAI o3-mini-high. Constrained by the availability or stabilization of API, we do not provide the performance of these newly released models. In the future, we will evaluate their long code understanding abilities on \method.

\ding{184} In our experiments, we only consider the long code with 0$\sim$128K tokens, although some LCLMs have supported longer context windows, \eg Claude-3-5-Sonnet with 200K context size and even Gemini-1.5-Flash with 1000K context size. We will continue to update and evolve our benchmark, in order to support \method to measure LCLMs on longer codes.


